Collective Model Intelligence Requires Compatible Specialization

In this work, we explore the limitations of combining models by averaging intermediate features, referred to as model merging, and propose a new direction for achieving collective model intelligence through what we call compatible specialization. Current methods for model merging, such as parameter and feature averaging, struggle to effectively combine specialized models due to representational divergence during fine-tuning. As models specialize to their individual domains, their internal feature representations become increasingly incompatible, leading to poor performance when attempting to merge them for new tasks. We analyze this phenomenon using centered kernel alignment (CKA) and show that as models specialize, the similarity in their feature space structure diminishes, hindering their capacity for collective use. To address these challenges, we investigate routing-based merging strategies, which offer more flexible methods for combining specialized models by dynamically routing across different layers. This allows us to improve on existing methods by combining features from multiple layers rather than relying on fixed, layer-wise combinations. However, we find that these approaches still face limitations when layers within models are representationally incompatible. Our findings highlight the importance of designing new approaches for model merging that operate on well-defined input and output spaces, similar to how humans communicate through language rather than intermediate neural activations.

==> future.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/future.pdf}  % Replace with your figure file
    \caption{Vision for collective intelligence: users can upload models $M(x)$, represented by the small colored rectangles, as well as tasks
$\{(x,y)\}$. The router dynamically organizes existing modules to solve the uploaded tasks. Once the task is solved, the modules are added back to the library, enabling reuse and continuous expansion of the system’s capabilities. This modular, collaborative approach facilitates efficient problem-solving and knowledge sharing across different domains.}
    \label{fig:future}  % Optional: Add a label for referencing
\end{figure}

==> loss.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/fig4.pdf}  % Replace with your figure file
    \caption{Validation cross-entropy loss (CE Loss) for math and coding models during finetuning. The math and coding models exhibit steady decreases in validation loss as they specialize on their respective tasks. In contrast, the performance of the merged model on a cross-domain task requiring both math and coding (activation interpolation) increasese gradually.}
    \label{fig:merging_loss_time}  % Optional: Add a label for referencing
\end{figure}

==> loss_vs_kernel.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/fig5.pdf}  % Replace with your figure file
    \caption{Merging performance plotted against CKA distance across checkpoints at different training timesteps in our cross domain task. The plot shows that as the CKA distance between model representations increases, merging performance tends to degrade. This suggests that larger representational differences between models correlate with higher loss, suggesting the importance of representational alignment in successful model merging.}
    \label{fig:CKA_vs_loss}  % Optional: Add a label for referencing
\end{figure}
